A Nonconvex Approach for Exact and Efficient Multichannel Sparse Blind Deconvolution

We study the multi-channel sparse blind deconvolution (MCS-BD) problem, whose task is to simultaneously recover a kernel $\mathbf a$ and multiple sparse inputs $\{\mathbf x_i\}_{i=1}^p$ from their circulant convolution $\mathbf y_i = \mathbf a \circledast \mathbf x_i $ ($i=1,\cdots,p$). We formulate the task as a nonconvex optimization problem over the sphere. Under mild statistical assumptions of the data, we prove that the vanilla Riemannian gradient descent (RGD) method, with random initializations, provably recovers both the kernel $\mathbf a$ and the signals $\{\mathbf x_i\}_{i=1}^p$ up to a signed shift ambiguity. In comparison with state-of-the-art results, our work shows significant improvements in terms of sample complexity and computational efficiency. Our theoretical results are corroborated by numerical experiments, which demonstrate superior performance of the proposed approach over the previous methods on both synthetic and real datasets.

==> sec/main_analysis.tex <==

In this section, we show that the underlying benign \emph{first-order geometry} of the optimization landscapes of \Cref{eqn:problem} \emph{enables} efficient and exact recovery using \emph{vanilla} gradient descent methods, even with \emph{random} initialization. Our main result can be captured by the following theorem, \revised{with details described in the following subsections.}
\begin{theorem}\label{thm:Main-all}
We assume that the kernel $\mb a$ is invertible with condition number $\kappa$, and $\Brac{\mb x_i}_{i=1}^p \sim \mc {BG}(\theta)$. Suppose $\theta \in \paren{\frac{1}{n} , \frac{1}{3} }$ and $\mu \leq c\min\Brac{ \theta, \frac{1}{\sqrt{n}} } $. Whenever
\begin{align}\label{eqn:sample-complexity-p}
  p \geq C \max\Brac{n , \frac{\kappa^8 }{ \theta \mu^2 \sigma_{\min}^2 } \log^4 n } \theta^{-2} n^4 \log^3(n) \log \paren{ \frac{ \theta n }{ \mu} },
\end{align}
w.h.p. the function \eqref{eqn:problem} satisfies certain regularity conditions \revised{(see \Cref{prop:regularity-main}), allowing us to design an efficient vanilla first-order method. In particular, with probability at least $\frac{1}{2}$, by using a random initialization, the algorithms provably recover} the target solution up to a signed shift with $\eps$-precision in a linear rate
\vspace{-0.05in}
   \begin{align*}
   	  \# Iter \;\leq \; C'\paren{ \theta^{-1}n^4 \log \paren{ \frac{1}{\mu} } + \log(np) \log\paren{ \frac{1}{\eps}} }.
   \end{align*}
\end{theorem}

\paragraph{Remark 1.} The detailed proofs are detained to Appendix \ref{app:geometry-main} and Appendix \ref{app:convergence}. In the following, we explain our results in several aspects.
\begin{itemize}[leftmargin=*]
	\item \emph{Conditions and Assumptions.} Here, as the MCS-BD problem becomes trivial\footnote{\edited{The problem becomes trivial when $\theta \leq 1/n$ because $\theta n= 1$ so that each $\mb x_i$ tends to be an one sparse $\delta$-function.}} when $\theta \leq {1}/{n}$, we only focus on the regime $\theta > {1}/{n}$. Similar to \cite{li2018global}, our result only requires the kernel $\mb a$ \edited{to be invertible} and sparsity level $\theta$ to be constant. In contrast, the method in \cite{wang2016blind} only works when the kernel $\mb a$ is spiky and $\Brac{\mb x_i}_{i=1}^p$ are very sparse $\theta \in \mc O(1/\sqrt{n})$, excluding most problems of interest.
	\item \emph{Sample Complexity.}  As shown in \Cref{tab:comparison}, our sample complexity $p \geq \wt{\Omega}(\max\Brac{n,{\kappa^8}/{\mu^2}}n^4)$ in \Cref{eqn:sample-complexity-p} improves upon the result $p \geq \wt{\Omega}(\max\Brac{n,\kappa^8}{n^8}/{\eps^8})$ in \cite{li2018global}. As aforementioned, this improvement partly owes to the similarity of the Huber-loss to $\ell^1$-loss, so that the Huber-loss is much less heavy-tailed than the $\ell^4$-loss studied in \cite{li2018global}, requiring fewer samples for measure concentration. Still, our result leaves much room for improvement --  we believe the sample dependency on $\theta^{-1}$ is an artifact of our analysis\footnote{The same $\theta^{-1}$ dependency also appears in \cite{sun2016complete,li2018global,bai2018subgradient,zhang2018structured,gilboa2018efficient}.}, and the phase transition in \Cref{fig:phase pn} suggests that $p \geq \Omega( \mathrm{poly}\log(n) )$ samples might be sufficient for exact recovery. 
	\item \emph{Algorithmic Convergence.} Finally, it should be noted that the number of iteration $\wt{O}\paren{ n^4 + \log\paren{{1}/{\eps} } } $ for our algorithm substantially improves upon that $\wt{\mc O}(n^{12}/\eps^2)$ of the noisy RGD in \cite[Theorem IV.2]{li2018global}. This has been achieved via a two-stage approach: (i) we first run $\mc O(n^4)$ iterations of vanilla RGD to obtain an approximate solution; (ii) then perform a subgradient method with linear convergence to the ground-truth. Moreover, without any noise parameters to tune, vanilla RGD is more practical than the noisy RGD in \cite{li2018global}.
\end{itemize}





%\zz{I think it's OK to not talk about $\theta$}

%Discuss about $p-\kappa$ trade-off, remove the discussion in Section 2.


%\subsection{A glimpse of high dimensional geometry}

\subsection{A glimpse of high dimensional geometry}\label{subsec:geometry}
\input{sec/geometry}


\subsection{From geometry to efficient optimization}\label{subsec:algorithm}
\input{sec/algorithm}



